Infusing Prompts with Syntax and Semantics

Despite impressive success, language models often generate outputs with flawed linguistic structure. We analyze the effect of directly infusing various kinds of syntactic and semantic information into large language models. To demonstrate the value of our proposals, we focus on the translation of natural language queries to SQL, in particular dealing with languages with less resources than English, to better investigate how much help we can get from low cost syntactic and semantic information. We show that linguistic analysis can significantly boost language models, to the point that we have surpassed previous best systems.

==> main.tex <==
\begin{abstract}
Despite impressive success, language models often generate outputs with flawed linguistic structure. We analyze the effect of directly infusing various kinds of syntactic and semantic information into large language models. To demonstrate the value of our proposals, we focus on the translation of natural language queries to SQL, in particular dealing with languages with less resources than English, to better investigate how much help we can get from low cost syntactic and semantic information. We show that linguistic analysis can significantly boost language models, to the point that we have surpassed previous best systems. 
% %
% Natural language to SQL is the task of translating a natural language request into a SQL query that answers the question from a specific database.
% With the recent advances in the deep learning and natural language processing areas, deep learning approaches for the task of translating natural language for SQL have flourished. Despite relevant results for important benchmarks T
% he results presented by these models in those benchmarks unlocked new heights. However, as models that also use transformers based language models (LMs) \cite{leivada2022dalle,yao2022structural}, they struggle with the interpretation of phrasal structures, which is vital for the correct translation of them, and consequently the user's intention conveyed by them, into the correct SQL query. We investigate the infusion of syntactic and semantic relations of the phrase into the input of Large Language Models (LLMs).
% %For languages other than English, or the models need to be trained with the new language, or the user needs to rely on a translator to make an inference with the model, having the burden of additional time and processing cost. 
% In our work, we focus  in languages other than English, as to make the inference of the model more accessible for speakers of these languages, without having to rely on translators: French, Spanish and Portuguese. 
% Our experiments were made for three languages (French, Spanish and Portuguese) and two language models, and show that syntactic and semantic information promotes a more effective and efficient fine-tuning, achieving state of the art results and high results after few training epochs.
% %considerably improves the quality of translations, and, in fact, make the training more effective and efficient
% %This document is a supplement to the general instructions for *ACL authors. It contains instructions for using the \LaTeX{} style files for ACL conferences.
% %The document itself conforms to its own specifications, and is therefore an example of what your manuscript should look like.
% %These instructions should be used both for papers submitted for review and for final versions of accepted papers.
\end{abstract}

\section{Introduction}

In this short paper we introduce techniques that infuse syntactic and semantic
information into large language models, and we show that relatively simple ideas
lead to key gains in performance. 
In essence, we infuse syntactic and semantic information in textual form, instead of changing computational paths as investigated in previous proposals. 

To be concrete, we focus on the translation
of natural language questions to SQL queries, using languages other than English
so as to face more challenging scenarios where one can really benefit from varied linguistic devices. 
We show that, at a relatively low cost, one can significantly boost the performance of language models --- for instance, we have been able to  surpass the previous state of art result on the Spider benchmark for Portuguese questions to SQL queries.
We hope these results will drive people to revisit syntactic and semantic information that can have as much effect as large amounts of data while consuming
less resources. 

The paper is organized as follows.
In Section~\ref{section:Background} we briefly go through relevant 
previous work;
in Section \ref{section:Proposal} we describe our proposals, and
in Section~\ref{section:exp} we describe our experiments.
Section~\ref{section:Conclusion} wraps up with some discussion and conclusions. 

% In the era of Big Data, in which we live, the production and consumption, for precise
% analysis, of a large volume of data is intense propelling human activities across a wide range of industries, ranging from banks to startups. As for the end users for the information derived from the a company's database, they are not only technical, but also business analysts, who do not necessarily understand the database querying concepts. Thus, these latter public rely on the technical people to gather the information needed from the database to make effective decisions. In order to make this process of gathering database information more accessible, specially for non-technical users, and quick, there has been interest in the development of natural language querying systems, namely natural language to SQL, which is a typical language to query data from relational databases.

% Natural language to SQL is the task of translating a natural language request into a SQL query that answers the question from a specific database. Many of the early efforts in this direction were rule-based \cite{nalir,athena}. These approaches recognize the schema terms in the natural language question and map the input to an underlying representation. This representation is then translated into a SQL format (abstract tree or even the proper SQL query). Although these models work well for targeted structures, they fall short in generalizing for questions that are not in their semantic coverage, relying in the width of this semantic coverage defined by manually defined rules. 

% With the recent advances in the deep learning and natural language processing areas, deep learning approaches have flourished. These proposals mainly formulate the problem as a translation task, training the networks with large amounts of question-SQL pairs, which are provided by datasets as WikiSQL \cite{zhong2017seq2sql} and Spider \cite{yu2019spider}. The results presented by these models in those benchmarks unlocked new heights. However, as models that also use transformers based language models (LMs) \cite{leivada2022dalle,yao2022structural}, they struggle with the interpretation of phrasal structures, which is vital for the correct translation of them, and consequently the user's intention, into the correct SQL query. 

%  despite the advances in the task of natural to SQL, for languages other than, this field does not follow this same fast pace. However, for languages other than English, the advances in the task of natural language to SQL do not follow this same fast pace. As far as we know, the latest work for this topic is \cite{Jos__2021}, which is the state of the art for the Portuguese language. An alternative to this problem could be the use of a translation module for the user question to English. Nevertheless, this approach would bind the use of the proper natural language to SQL model to an external translation API or to a translation model from a given language to English, either way it would burden the usage of the model with an additional time cost to run the translation from language to language, with the former proposal having to send information (which might be sensitive for some use cases) to an external server. Hence, \citet{Jos__2021} use an already translated version of Spider dataset to Portuguese to train the model, achieving 0.664 of exact-set match without values in the benchmark, which is far though from the English standard.

% In this paper,  we investigate infusing semantic and syntactic relations into language models. In particular, we train models for the natural language to SQL task with the raw question, in  language other than English, with the syntactic information about the phrase and phrase in a language other than English and with the phrase and its semantic representation. All of these models are trained using a language other than English. Contrary to other proposals that modify a network's architecture to capture such syntactic information, we present it in raw text format. We show that providing syntactic and semantic relations is important for the model. Notably, the accuracies were higher and achieved the state of the art for the languages used in the Spider benchmark. 

% %The templates include the \LaTeX{} source of this document (\texttt{acl\_latex.tex}),
% %the \LaTeX{} style file used to format it (\texttt{acl.sty}),
% %an ACL bibliography style (\texttt{acl\_natbib.bst}),
% %an example bibliography (\texttt{custom.bib}),
% %and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Background and Related Work}\label{section:Background}

There are a number of techniques that aim at infusing morphological/syntactic/semantic information into language models (LMs).
\citeauthor{Punyakanok2008} (\citeyear{Punyakanok2008}) is an early 
example of syntactic infusion in role labeling (without transformers). 
Other   efforts  mix classic linguistic
results within learning techniques \cite{sogaard-goldberg-2016-deep}.
%Such combinations have been proven valuable in  Recurrent Neural Networks (RNNs) \cite{futrell-etal-2019-neural,wilcox-etal-2019-structural}.
%
%There has been recent interest in inserting symbolic information into LMs during training time. 
\citeauthor{Shiv2019} (\citeyear{Shiv2019}) use a positional
embedding that exploits relations in a syntax trees, so as to get some of
the syntactic structure into an LM. Clearly this requires changes to the
original transformer model. Another effort, by 
\citeauthor{Qian2021} (\citeyear{Qian2021}), modifies the training of
the LM by asking the model to predict not only words but also parse trees.
%containing morphological information. 

Morphological parse trees have also been used during training;
\citeauthor{selfattentionBai2021} (\citeyear{selfattentionBai2021}) have
self-attention modules for each relation from a morphological tree.
%, with applications for instance in sentiment analysis and natural language inference.
And morphological trees have  been mapped to vectors by embeddings \cite{zanzotto-etal-2020-kermit},
with tests on encoder-only models for classification tasks.
\citeauthor{currey2019incorporating} (\citeyear{currey2019incorporating}) enhance
translation performance  by infusing morphology trees as input to trained encoders, and also improve translation with encoder-decoder models by pre-training the model on a parsing task. 
\citeauthor{sg-net} (\citeyear{sg-net}) uses a network to insert morphological relations
into the self-attention mechanism of a LM.
%, with experiments in machine reading comprehension. 
Regarding the transformer's attention mechanism, \cite{9303437} uses the information of the words related to each other in  the attention mechanism.

Structures beyond morphological relations have also been infused
into LMs. For instance, \citeauthor{bert-parse} (\citeyear{bert-parse}) use a graph similar to
the Abstract Meaning Representation (AMR) of the input  during training
for an encoder architecture (with experiments in various classification tasks). 
%We also benefit from AMR in our proposed techniques.
Another work that relies on syntactic relations, by \citeauthor{nmt} (\citeyear{nmt}),
introduces  embeddings for syntactic features and then combine those embeddings, and positional
encodings. (Note: we also
infuse syntactic information but we rely on a single
embedding and do not make changes to positional
encodings nor to   architectural elements of the LM.)

We now add a few comments about the (very large!) literature
on natural language to SQL translation, referred to as NL2SQL. 
Early efforts in NL2SQL were
rule-based \cite{nalir,athena}, but now the best systems rely on deep networks
learned with large datasets such as WikiSQL \cite{zhong2017seq2sql} and
Spider \cite{yu2019spider}. However, transformers still struggle with
phrasal structures, for instance ones that carry user intentions.
These difficulties are particularly acute in languages other than
English for which datasets with examples are small. Even though one can always
translate to English and then call an English translator to SQL, this approach
increases translation time and   cost, and obviously depends on
the first translation that may also be poor. 
In addition, a previous study \cite{jose2021mrat}, \cite{jose2023multilingual}
on NL2SQL in Portuguese has found that a single multilingual transformer 
works better than a translation to English (followed by a  
English-trained transformer). 

% The translation of natural language questions to SQL, often referred to as NL2SQL,
% is a promising task that can help many individuals who are not proficient in SQL
% and yet have to look for information in databases. Early efforts in NL2SQL were
% rule-based \cite{nalir,athena}, but now the best systems rely on deep networks
% learned with large datasets such as WikiSQL \cite{zhong2017seq2sql} and
% Spider \cite{yu2019spider}.
% However, transformer-based NL2SQL still struggles with the interpretation of phrasal 
% structures that carry significant meaning, often indicating the user's
% intentions. These difficulties are particularly acute in languages other than
% English for which datasets with examples are small. Even though one can always
% translate to English and then call an English translator to SQL, this approach
% increases translation time and effort (and cost), and obviously depends on
% the first translation that may also be poor. We show here that excellent NL2SQL
% systems can be obtained by resorting to the kind of syntactic and semantic
% information that one can easily obtain with existing linguistic tools. 
 
%  However, for languages other than English, the advances in the task of natural language to SQL do not follow this same fast pace. As far as we know, the latest work for this topic is \cite{Jos__2021}, which is the state of the art for the Portuguese language. An alternative to this problem could be the use of a translation module for the user question to English. Nevertheless, this approach would bind the use of the proper natural language to SQL model to an external translation API or to a translation model from a given language to English, either way it would burden the usage of the model with an additional time cost to run the translation from language to language, with the former proposal having to send information (which might be sensitive for some use cases) to an external server. Hence, \citet{Jos__2021} use an already translated version of Spider dataset to Portuguese to train the model, achieving 0.664 of exact-set match without values in the benchmark, which is far though from the English standard.
 
There have been efforts that employ parsers within NL2SQL. For instance, \cite{Yaghmazadeh2017} \cite{iyer2017learning} parse the input   and maps it to a representation near, such as the skeleton, or even the proper SQL query. Therefore neither of them actually applies linguistic analysis of the phrase structure. On the other hand, \cite {nalir}, even though relying on a framework that requires human feedback for the generated queries, makes use of the morphological tree of the phrase as an intermediate representation of the user query to generate by rule-mapping the query, not using transformers. Neither of these approaches infuse formal phrase structure information into transformers, nor  use  the input syntax or semantics, as we do in our method. %nor the use of the particular type of information about the phrase which we use in our method, namely syntax and semantics



\section{Infusing syntactic and semantic information}\label{section:Proposal}

%%%%%%%%%%%%%%%%
%%% TO ANALYZE: 
% In tasks sensitive to input phrases, that is, tasks in which a little modification in the input phrase can produce a perceptive difference in the output, it is important for the model to capture and understand the relations between the terms of the phrase as to generate the correspondent output, reflecting them, and consequently, the user's intention that they convey as a whole.%ultimately
% For instance, in the task of translation from natural language to natural language, adjectives are supposed to only modify corresponding nouns, and such connections must be respected in translated output. However, transformers not always are capable of interpreting correctly these relations, resulting in outputs that flaw, or do not translate or represent, the relations required by the user's phrase. %which impede them of translating it to the output, which results in a output that flaws the user's intention

Intuitively, one might think that syntactic information is bound
to improve LMs; however, it is not easy to see how to infuse
such information in ways that actually make a positive difference 
at low cost.
We explore a direct strategy where syntactic information is 
  fed as part of the LM input. To do so, we 
concatenate syntactic information with the raw input text. 
We use such enlarged input  during
training and inference, even though it is possible to produce
outputs without enlarging the input (with syntactic and semantic information)
 during inference.
Thus we do not have to change the architecture of the LM of choice.

The resulting pipeline is depicted in Figure \ref{figure:Pipeline}:
the input goes through syntatic and semantic analysis, and then it
is concatenated with the result of that analysis; the concatenated
text along with the schema related to the request goes to the LM. 


\begin{figure}[t]
\centering
\begin{tikzpicture}
\node[white,draw,rectangle,rounded corners,fill=violet] (input) at (1,1) {Input};
\node[draw,rectangle,fill=yellow] (parser) at (3,1.7) {Parser};
\node[draw,rectangle,fill=yellow] (LM) at (5,1) {LM};
\node[white,draw,rectangle,rounded corners,fill=violet] (output) at (7,1) {Output};
\draw[->,>=latex] (input)--(parser);
\draw[->,>=latex] (input)--(LM);
\draw[->,>=latex] (parser)--(LM);
\draw[->,>=latex] (LM)--(output);
\end{tikzpicture}
\caption{The pipeline, from input to output.}
\label{figure:Pipeline}
\end{figure}

We rely on two types of information about the phrase: dependency trees \cite{jurafsky}, representing the syntax, and AMR data, for the semantic. The \textit{Abstract Meaning Representation} (AMR) is a semantic representation framework that captures the meaning of a sentence 
through a directed acyclic graph where nodes correspond to concepts 
or entities, and edges represent various  relationships 
between them. Concepts are typically abstract and 
language-independent in AMR, allowing for a higher level of semantic 
generalization. The relationships between concepts capture roles, 
attributes, and dependencies.
%Syntactic information can be extracted using a parser, and the recent evolution of natural language parsers has been so significant that their output can surely be expected to help LMs.

To translate a dependency tree into running text, we follow a proposal by \citeauthor{Li2021} (\citeyear{Li2021}): for each word, we initiate the sentence with [row] and separate each output of the parser by ``;'', if the word does not have any child, we end  the sentence with </none>.
For instance, suppose an input sentence is as follows for a translation from French to SQL: ``Inscrivez l'année de création, le nom et le budget de chaque département.'' The text produced out of the dependency tree for this input is:
\begin{quote} \small
Inscrivez l'année de création, le nom et le budget de chaque département. [row] year; dobj [row] name; conj [row] budget; conj [row] department; pobj    
\end{quote}
  
To infuse semantic information, we turn  AMR graphs to   text by  removing spaces and relying on AMR brackets  %, as we operated with " ; ",  
to separate the parser's output, in order to teach the model how to make the correct associations in   PropBank notation. 
For instance, if we have the same input sentence as above, the running text
produced out of the AMR analysis is
\begin{quote} \small
    Inscrivez l'année de création, le nom et le budget de chaque département. (l / list - 01 :ARG1 (a / and :op1 (y / year :time - of (c / create - 01 :ARG1 (d / department :mod (e / each)))) :op2 (n / name :poss d) :op3 (b / budget :poss d)))
\end{quote}
%insert amr

We adopt the RESDSQL framework for NL2SQL \cite{li2022resdsql}. In this framework, a trained encoder model (Roberta \cite{liu2019roberta}), given the user's request, selects the most relevant tables and columns accordingly, and presents only them along the user question to the transformer. Besides, in RESDSQL, the language model used to generate SQL first decodes the SQL structure from the structure, without assigning values, and then the language model generates the complete SQL output. 


\begin{table*}\small
  \centering
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{French}} &  \multicolumn{4}{c|}{\textbf{Spanish}}& \multicolumn{4}{c|}{\textbf{Portuguese}}\\
    % \hline
    % \textbf{Inactive Modes} & \textbf{Description}\\
    \cline{2-13}
    & \textbf{EM} & \textbf{EX}  & \textbf{v1} & \textbf{v2} & \textbf{EM} & \textbf{EX} & \textbf{v1} & \textbf{v2} &\textbf{EM}  &\textbf{EX}& \textbf{v1} & \textbf{v2}\\
    %\hhline{~--}
    \hline
    T5 without info  & 0.612 & 0.618  & - & -  & 0.582 & 0.612  & - & -  &  0.550 & 0.575  & - & - \\ \hline
    T5 with syntax & 0.623  & 0.649 & 1.8 & 5.0 &  0.616 & 0.631 & 5.8 & 3.1 & 0.591 & 0.625  & 7.4 & 7.6   \\
      \hline
    T5 with AMR  & 0.640 & 0.693 & 4.6  & 12.1 & 0.635 & 0.691 & 9.14  & 12.9 & 0.639 & 0.682 & 16.2 & 18.5 \\ 
      \hline
      T5 with syntax + AMR  & 0.638 & 0.684 &   &  & 0.639  & 0.679 &   &  &  &  &  &  \\ 
      \hline
      Bart without info & 0.199 & 0.199 & - & - & 0.199 & 0.199 & - & - & 0.182  & 0.181 & - & -  \\ \hline
      Bart with syntax & 0.234 & 0.249 &  17.6 & 25.0 & 0.223 & 0.236 & 12.1  & 18.6 & 0.216 & 0.221   &  40.2 & 37.3 \\
      \hline
      Bart with AMR & 0.215 & 0.225 & 8.0 & 13.0 & 0.242 & 0.262 & 21.6 & 31.7 & 0.222  & 0.245  & 40.2 & 52.4  \\
    \hline
    Bart with syntax + AMR & 0.269  & 0.286 &  &  & 0.255 & 0.282 &  &  & 0.287  &  0.311 &  &   \\
    \hline
    %Third condition & TBD & TBD & &  1200 & 1200 &  & 1200 &  1200 &  \\ \hline
  \end{tabular} 
  
%%%%%%%%%%%% Spanish: T5 -   
%%%%%%%%%%%%          Bart - 128  aval s07

%%%%%%%%%%%% 
%%%%%%%%%%%% Portuguese: T5 - 32 and 128 epochs arandu train aval
%%%%%%%%%%%%           
\vspace*{1ex}

  \centering
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{French}} &  \multicolumn{4}{c|}{\textbf{Spanish}}& \multicolumn{4}{c|}{\textbf{Portuguese}}\\
    % \hline
    % \textbf{Inactive Modes} & \textbf{Description}\\
    \cline{2-13}
    & \textbf{EM} & \textbf{EX}  & \textbf{v1} & \textbf{v2} & \textbf{EM} & \textbf{EX} & \textbf{v1} & \textbf{v2} &\textbf{EM}  &\textbf{EX}& \textbf{v1} & \textbf{v2}\\
    %\hhline{~--}
    \hline
    T5 without info  & 0.618  & 0.632  & - & -  & 0.591  & 0.618  & - & - &  0.586 & 0.602 & - & - \\ \hline
    T5 with syntax & 0.657  & 0.673 & 6.3 & 6.5 &  0.631 & 0.636 & 6.8 & 2.9  & 0.630  & 0.649  & 7.4 & 7.9  \\
      \hline
    T5 with AMR  & 0.669 & 0.700 &  8.2 & 10.8  & 0.653  & 0.687  & 10.5 & 11.2 & 0.653  &   0.687  & 11.4 & 14.1 \\ 
      \hline
      T5 with syntax + AMR  & 0.652 & 0.695 &   &  & 0.651 & 0.708 &   &  &  &  &  &  \\ 
      \hline
      Bart without info & 0.184 & 0.184 & - & - & 0.197 & 0.199 & - & - & 0.163  & 0.171 & - & -  \\ \hline
      Bart with syntax &  0.238 & 0.240  & 29.3  & 30.4  & 0.218  & 0.220  & 10.7  & 10.6 & 0.218 & 0.222   &  33.1 & 29.9 \\
      \hline
      Bart with AMR & 0.227  & 0.240 & 23.4 & 30.4 & 0.210 & 0.224    & 6.6  & 12.6 & 0.189 & 0.196 & 15.9  & 14.6 \\
    \hline
    Bart with syntax + AMR & 0.279 & 0.299 &  &  &  &  &  &  &  0.285 & 0.305  &  &   \\
    \hline
    %Third condition & TBD & TBD & &  1200 & 1200 &  & 1200 &  1200 &  \\ \hline

  \end{tabular}
  %\vspace*{-1ex}
\caption{Model performance after training for 32 (top) and 128 (bottom) epochs.}  \label{table:theTable}
\end{table*}
%%%%%%% chinese
\begin{table*}\small
  \centering
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{Chinese}} &  \multicolumn{4}{c|}{\textbf{Spanish}}& \multicolumn{4}{c|}{\textbf{Portuguese}}\\
    % \hline
    % \textbf{Inactive Modes} & \textbf{Description}\\
    \cline{2-13}
    & \textbf{EM} & \textbf{EX}  & \textbf{v1} & \textbf{v2} & \textbf{EM} & \textbf{EX} & \textbf{v1} & \textbf{v2} &\textbf{EM}  &\textbf{EX}& \textbf{v1} & \textbf{v2}\\
    %\hhline{~--}
    \hline
    T5 without info  & 0.094 & 0.251  & - & -  & 0.582 & 0.612  & - & -  &  0.550 & 0.575  & - & - \\ \hline
     mT5 without info  & 0.522 & 0.678  & - & -  & 0.582 & 0.612  & - & -  &  0.550 & 0.575  & - & - \\ \hline
    T5 with syntax & 0.623  & 0.649 & 1.8 & 5.0 &  0.616 & 0.631 & 5.8 & 3.1 & 0.591 & 0.625  & 7.4 & 7.6   \\
      \hline
    T5 with AMR  & 0.640 & 0.693 & 4.6  & 12.1 & 0.635 & 0.691 & 9.14  & 12.9 & 0.639 & 0.682 & 16.2 & 18.5 \\ 
      \hline
      T5 with syntax + AMR  & 0.638 & 0.684 &   &  & 0.639  & 0.679 &   &  &  &  &  &  \\ 
      \hline
      Bart without info & 0.199 & 0.199 & - & - & 0.199 & 0.199 & - & - & 0.182  & 0.181 & - & -  \\ \hline
      Bart with syntax & 0.234 & 0.249 &  17.6 & 25.0 & 0.223 & 0.236 & 12.1  & 18.6 & 0.216 & 0.221   &  40.2 & 37.3 \\
      \hline
      Bart with AMR & 0.215 & 0.225 & 8.0 & 13.0 & 0.242 & 0.262 & 21.6 & 31.7 & 0.222  & 0.245  & 40.2 & 52.4  \\
    \hline
    Bart with syntax + AMR & 0.269  & 0.286 &  &  & 0.255 & 0.282 &  &  & 0.287  &  0.311 &  &   \\
    \hline
    %Third condition & TBD & TBD & &  1200 & 1200 &  & 1200 &  1200 &  \\ \hline
  \end{tabular} 
  
%%%%%%%%%%%% Spanish: T5 -   
%%%%%%%%%%%%          Bart - 128  aval s07

%%%%%%%%%%%% 
%%%%%%%%%%%% Portuguese: T5 - 32 and 128 epochs arandu train aval
%%%%%%%%%%%%           
\vspace*{1ex}

  \centering
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{French}} &  \multicolumn{4}{c|}{\textbf{Spanish}}& \multicolumn{4}{c|}{\textbf{Portuguese}}\\
    % \hline
    % \textbf{Inactive Modes} & \textbf{Description}\\
    \cline{2-13}
    & \textbf{EM} & \textbf{EX}  & \textbf{v1} & \textbf{v2} & \textbf{EM} & \textbf{EX} & \textbf{v1} & \textbf{v2} &\textbf{EM}  &\textbf{EX}& \textbf{v1} & \textbf{v2}\\
    %\hhline{~--}
    \hline
    T5 without info  & 0.618  & 0.632  & - & -  & 0.591  & 0.618  & - & - &  0.586 & 0.602 & - & - \\ \hline
    T5 with syntax & 0.657  & 0.673 & 6.3 & 6.5 &  0.631 & 0.636 & 6.8 & 2.9  & 0.630  & 0.649  & 7.4 & 7.9  \\
      \hline
    T5 with AMR  & 0.669 & 0.700 &  8.2 & 10.8  & 0.653  & 0.687  & 10.5 & 11.2 & 0.653  &   0.687  & 11.4 & 14.1 \\ 
      \hline
      T5 with syntax + AMR  & 0.652 & 0.695 &   &  & 0.651 & 0.708 &   &  &  &  &  &  \\ 
      \hline
      Bart without info & 0.184 & 0.184 & - & - & 0.197 & 0.199 & - & - & 0.163  & 0.171 & - & -  \\ \hline
      Bart with syntax &  0.238 & 0.240  & 29.3  & 30.4  & 0.218  & 0.220  & 10.7  & 10.6 & 0.218 & 0.222   &  33.1 & 29.9 \\
      \hline
      Bart with AMR & 0.227  & 0.240 & 23.4 & 30.4 & 0.210 & 0.224    & 6.6  & 12.6 & 0.189 & 0.196 & 15.9  & 14.6 \\
    \hline
    Bart with syntax + AMR & 0.279 & 0.299 &  &  &  &  &  &  &  0.285 & 0.305  &  &   \\
    \hline
    %Third condition & TBD & TBD & &  1200 & 1200 &  & 1200 &  1200 &  \\ \hline

  \end{tabular}
  %\vspace*{-1ex}
\caption{Model performance after training for 32 (top) and 128 (bottom) epochs.}  \label{table:theTable}
\end{table*}


 
\section{Experiments}\label{section:exp}

Our experiments investigate whether syntactic and semantic information in the task of translating natural language to SQL. This task is rather sensitive: a small
mistake in understanding the user intents can lead to seriously incorrect SQL queries. Hence one might expect linguistic analysis to be valuable. 

%%%%%%%%%%%%
%XXXX
% In this study, \citet{Jos__2021} propose the use of a multilingual transformer encoder-decoder architecture in the task of translating from natural languages others than English to their queries, including French and Portuguese. %, and in \citealt{jose2023multilingual} it is also used a module to reduce the schema (only  tables) in the input of the transformer.
 % We use in our training the translated versions of the Spider dataset \cite{yu2019spider} that were generated in this study. The translated dataset has three splits: training (with 7000 question/answer pairs), training others (with 1659 question/answer pairs) and dev (1034 question/answer pairs), for validation. %, using the \cite{RAT} proposal
%%%%%%%%%%%%%%%%%%%%

As English NL2SQL systems have already received myriad improvements (so that any individual technique is bound to have minimal impact), we worked with other languages so as to better
grasp the absolute value of our proposals. We have focused on French/Spanish/Portuguese translation to SQL. 
We employed translated versions of the Spider (under the CC BY-SA 4.0 license) dataset for training and testing.

Our experiments used Bart base \cite{lewis2019bart} and T5 base \cite{raffel2023exploring}
as LLMs. 
Dependency trees and AMR graphs have been generated by the Spacy parser and amrlib, respectively. For fine-tuning the base models, the experiments were conduced on 2 GPUs NVidia GeForce RTX 3090 24 GB. For the specific fine-tuning of a T5 with 3 billion parameters for Portuguese, a single A100 GPU with 80 GB was used.
All models were trained using the AdaFactor optimizer, with a learning rate of 1e-4, batch size of 8 and gradient descent after two step. 
Our code and resulting models will be made publicly available in case the present
text is accepted for publication, under the CC BY-SA 4.0 license.

We evaluated our models using  exact-set-match and execution accuracy.
These metrics are rather complementary, as exact-set-match may overlook more false negatives (one query might be the answer, even though not   the golden one), whereas execution accuracy may overlook more false positives (a value might be the one generated by the golden query, nonetheless by another term in the table, not the one referenced by the golden query). 

To understand the impact of syntactic and semantic information of the input in a model performance and its relevance during training,  we trained, for each language, a Bart model with the raw versions of the corresponding (translated) version of Spider, a model with the syntactic information and one with the semantic information infused. 
We then did the exact same set of training runs for the T5 models. Thus we
generated six distinct language models per natural language.
Using this scheme, we were able to compare   the results for the training without  any added linguistic information (raw dataset), solely with syntax infused, and solely  with semantics infused. 

Also,   we repeated the set of experiments described in the previous paragraph both for 32 and for 128 training epochs. With these two numbers of training epochs, operating with the same data and language model,   we were able to evaluate the   relevance of the information presented to the  progress of  the training process itself. 

Table  \ref{table:theTable} (top) conveys the results for the translations for the different languages of the corpus, for 32 epochs, while Table \ref{table:theTable} (bottom) presents the results of the models trained for 128 epochs with French, Spanish and Portuguese, respectively. The "EM" and "EX" columns contain values of exact-set match and execution accuracy respectively. 
%%%% HERE:
The v1 and v2 columns contain, respectively, the relative variation between the produced model's exact-set match accuracy and the base model exact-set match accuracy, and the relative variation between the produced model's execution accuracy and the base model  execution accuracy, in percentages.

The tables show that the infusion of syntactic and semantic information is valuable during training. Models that were fed during training with the input phrase  syntax or semantic structure displayed higher performance than the corresponding models without any linguistic information, regardless of the language model, for every natural language we tried. Also, this can be verified  both in the lower number of epochs and in the higher number of epochs.  In most experiments, the models that received  semantic information had the higher scores. Thus we can see that syntactic and semantic information lead to better scores.

In addition, syntactic and semantic information accelerate training. Even when trained only for 32 epochs, models with syntactic or semantic information achieve higher results than models without any such information but trained with four times more epochs (that is, with 128 epochs). Therefore, the infusion not only attains better performance within a given number of training epochs, but it also attains a given performance with a smaller number of epochs. Particularly, we were able to surpass the state of the art when training the models using the T5 architecture with 3 billion parameters and Nat SQL \cite{gan2021natural} as intermediate representation of the user's input and the corresponding SQL query, with 0.752 in exact-set match and 0.804 in execution accuracy --- this is a gain of 9.5\% in exact-set match against the state of the art (note that state of art results in the literature did not report  execution accuracy).  %effectiveness and efficiency 

We also note   that, comparing the performance of a model to its counterpart in the parallel group of training epochs (keeping same architecture and for the same language but training for a different number of epochs), the models infused with syntactic or semantic information trained for 32 epochs had values for both metrics near the values from their counterparts trained for 128 epochs. This suggests an expressive gain in training efficiency, allowing results near the values one would get after training the model for 128 epochs only after 32 epochs of training with syntax or semantics. This presents a reduction in the time cost of training the model, as well as in the energy consumed for it.
 

% \begin{table}\small
%   \centering
%   \renewcommand{\arraystretch}{1.2}
%   \begin{tabular}{|p{1.6cm}|c|c|c|c|c|c|}
%     \hline
%     \!\multirow{\textbf{Model}}\! & \multicolumn{2}{c|}{\textbf{French}} &  \multicolumn{2}{c|}{\textbf{Spanish}}& \multicolumn{2}{c|}{\textbf{Portuguese}}\\
%     % \hline
%     % \textbf{Inactive Modes} & \textbf{Description}\\
%     \cline{2-7}
%     &  \!\textbf{EM}  &  \!\textbf{EX}   &   \!\textbf{EM}  &  \!\textbf{EX} &  \!\textbf{EM}  &  \!\textbf{EX}  \\
%     %\hhline{~--}
%     \hline
%     \!T5 (no  info)\!  & \!0.61  &  \!0.62   &  \!0.58  &  \!0.61  &  \!0.55  &  \!0.58  \\ \hline
%     \!T5 + syntax\! &  \!0.62  & \!0.65  &   \!0.62  &  \!0.63 &  \!\!0.59 &  \!0.63 \\ \hline
%     \!T5 + AMR\! & \!0.64  &  \!0.69  &    \!0.64  &  \!0.69 &  \!0.64 &  \!0.68 \\ \hline
%     \!Bart (no info)\! &  \!0.20 &   0.20  &  \!0.20  &  \!0.20 &  \!0.18  &  \!0.18  \\ \hline
%     \!Bart + syntax\! &  \!0.23  &  \!0.25 &  \!0.22  &  \!0.24   &  \!0.22  &  \!0.22     \\
%       \hline
%     \!Bart + AMR\! & \!0.21  &  \!0.23  & \!0.24  &  \!0.26  &  \!0.22   &  \!0.25   \\
%     \hline
%   \end{tabular}

% \vspace*{1ex}

%   \centering
%     \begin{tabular}{|p{1.6cm}|c|c|c|c|c|c|}
%     \hline
%     \!\multirow{\textbf{Model}}\! & \multicolumn{2}{c|}{\textbf{French}} &  \multicolumn{2}{c|}{\textbf{Spanish}}& \multicolumn{2}{c|}{\textbf{Portuguese}}\\
%     % \hline
%     % \textbf{Inactive Modes} & \textbf{Description}\\
%     \cline{2-7}
%     & \!\textbf{EM} & \!\textbf{EX}  &  \!\textbf{EM} & \!\textbf{EX} & \!\textbf{EM} & \!\textbf{EX}\\
%     %\hhline{~--}
%     \hline
%     \!T5 (no  info)\!   & \!0.62  & \!0.63  & \!0.59  & \!0.62 & \!0.59 & \!0.60  \\ \hline
%      \!T5 + syntax\! & \!0.66  & \!0.67 &  \!0.63 & \!0.64 &  \!0.63  & \!0.65  \\ \hline
%     \!T5 + AMR\! & \!0.67 & \!0.70 &   \!0.65  & \!0.69 & \!0.65  &   \!0.69  \\ \hline
%     \!Bart (no info)\! & \!0.18 & \!0.18 & \!0.20 & \!0.20 & \!0.16  & \!0.17  \\ \hline
%     \!Bart + syntax\! &  \!0.24 & \!0.24 & \!0.22  & \!0.22  & \!0.22 & \!0.22    \\
%       \hline
%     \!Bart + AMR\! & \!0.23  & \!0.24 & \!0.21 & \!0.22  & \!0.19 & \!0.20  \\
%     \hline
%     %Fourth condition & TBD & TBD &   1200 & & 1200 & \\ \hline
%   \end{tabular}
%   \caption{Model's performance after training for 32 (top) and 128 (bottom) epochs.}
%   \label{table:theTable}
% \end{table}



\section{Conclusion}\label{section:Conclusion}

This is a short paper with a concise message: Syntactic and semantic information
should be used together with LLMs! The former can improve the latter, at low cost,
and in fact linguistic analysis can mitigate the need for ever larger annotated datasets.
This sort of message has been pursued in previous work, but we feel that we have here
described strategies that are simpler to apply, and that seem to be more effective.
%%
It should be emphasized that we do not
require changes in inner components of transformers (such as positional embeddings,
self attention layers, etc). In fact,  it is not even necessary to change the inputs
at inference time --- even though we have shown that adding syntact and semantic
information at inference time, and not only during training, is rather valuable.

Our experiments show that syntactic and semantic infusion helps in NL2SQL from
three natural languages, often
in a smaller number of training epochs. The representation that made the best contribution
was the one based on AMR graphs, even though dependency trees are also valuable.
%
% From the experiments ranging for three languages and two transformer architectures, %the results are concordant and follow the same pattern for all languages and almost for all architectures, which allows us to make the conclusion that the models benefit form the syntactic and semantic infusion
% we can conclude that the syntactic and semantic information infusion is relevant for the transformer model in the task. Our proposed technique enables the models trained with this knowledge for multiple languages different from English to achieve higher performance than would be seen with the baseline results, and for cases even in a fewer number of training epoch. Proof of this, with the work we have achieved a new state of the art for the Portuguese models in the task. Also, models trained with this knowledge achieve similar results near the ones that they achieve when trained for far more epochs (32 has results near the ones generated after training for 128 epochs), which suggests efficiency gain.
% Also, the proposal do not require changes in inner structures (such as positional embedding, self-attention, etc), and they work in a plug and play fashion: albeit being trained with the syntactic or semantic information in the input, the user at inference time is not required to pass this information as input (although the best results are guaranteed when the inference is made as was in training, with the knowledge). Among the different types of knowledge about the phrase we have examined -- dependency trees and AMR graphs, representing the syntactic type and semantic type, respectively -- the latter type has led to best results in general.
%
We close with two key points that our experiments indicate about our proposals.
Effectiveness: the positive value of training transformers with 
syntactic and semantic information, at least for languages that are not English, without   retraining the models (linguistic analysis led models
to attain higher performance than possible otherwise).
Efficiency: syntactic and semantic information do accelerate the training process,
enabling models to reach target performance levels in fewer training epochs.
